Some Results on the Functional Decomposition of Polynomials

If g and h are functions over some field, we can consider their composition f = g(h). The inverse problem is decomposition: given f, determine the ex- istence of such functions g and h. In this thesis we consider functional decom- positions of univariate and multivariate polynomials, and rational functions over a field F of characteristic p. In the polynomial case, "wild" behaviour occurs in both the mathematical and computational theory of the problem if p divides the degree of g. We consider the wild case in some depth, and deal with those polynomials whose decompositions are in some sense the "wildest": the additive polynomials. We determine the maximum number of decompositions and show some polynomial time algorithms for certain classes of polynomials with wild decompositions. For the rational function case we present a definition of the problem, a normalised version of the problem to which the general problem reduces, and an exponential time solution to the normal problem.

==> Mchardefs.tex <==
%
% Math character definitions:
%
\def\bull{{$\bullet$}}
\def\nats{{\Bbb N}}
%\def\Nats{{\Bbbla N}}
\def\ints{{\Bbb Z}}
%\def\Ints{{\Bbbla Z}}
\def\reals{{\Bbb R}}
\def\rats{\hbox{$\Bbb Q$}}
%\def\Rats{{\Bbbla Q}}
\def\cmplx{{\Bbb C}}
%\def\Cmplx{{\Bbbla C}}
\def\bool{{\Bbb B}}
\def\gf{{\Bbb F}}
\def\GF{\mathord{\rm GF}}
\def\gfc{{\overline{{\Bbb F}}}}
%\def\GFC{{\overline{{\Bbbla F}}}}
\def\setmid{{\,\mid\,}}
\def\setsep{{\mskip4mu:\mskip4mu}}
\def\eqdef{\mathrel{\buildrel {\rm def} \over =}}
\def\gal{\mathop{\rm Gal}}
\def\cont{\mathop{\hbox{cont}}}
\def\disc{\mathop{\rm disc}}
\def\rank{\mathord{\rm rank}}
\def\Span{\mathord{\rm span}}
\def\diag{\mathord{\rm diag}}
\def\rad{\mathop{\rm Rad}}
\def\norm{\mathop{\rm norm}}
\def\adj{\mathop{\rm adj}}
\def\charpoly{\mathord{\rm char}}
\def\minpoly{\mathord{\rm min}}
\def\ord{\mathop{\rm ord}}
\def\Ord{\mathop{\rm Ord}}
\def\End{\mathop{\rm End}}
\def\prob{\mathop{\rm Prob}}
\def\rem{\mathop{\rm rem}}
\def\res{\mathop{\rm res}}
\def\lcm{\mathop{\rm lcm}}
\def\Gcd{\mathord{\rm gcd}}
\def\divi{\mathop{\rm div}}
%\def\softO{{\widetilde O}}
\def\softO{{O\,\tilde{}\,}}
\def\nequiv{{\mathrel{\hbox{$\mskip4mu\not\equiv\mskip4mu$}}}}
\def\divs{{\mskip3mu|\mskip3mu}}
\def\ndivs{\nmid}
\def\nin{{\mathrel{\hbox{$\mskip4mu\not\in\mskip4mu$}}}}
\def\li{\mathop{\rm li}}
\def\re{\mathop{\rm Re}}
\def\im{\mathop{\rm Im}}
\def\th{{\hbox{\small th}}}
%\font\fivsf  = cmss10  scaled 490 
\def\trans{t}
\def\Tr{\mbox{Tr\,}}
\def\Null{\mbox{Null\,}}
\def\MM{\mathord{\mskip1mu{\rm MM}}}
\def\M{\mathord{\mskip1mu{\rm M}}}
\def\D{\mathord{\mskip1mu{\rm D}}}
\def\floor#1{{\left\lfloor #1 \right\rfloor}}
\def\ceil#1{{\left\lceil #1 \right\rceil}}
\def\jac#1#2{{\left({{#1}\over{#2}}\right)}_{\hbox{\tiny J}}}
\def\vstrut#1{\rule{0pt}{#1}}
\def\hstrut#1{\rule{#1}{0pt}}
\def\sfE{{\sf E}}
\def\sfF{{\sf F}}
\def\sfK{{\sf K}}
\def\sfL{{\sf L}}
\def\nonzero{\setminus\{0\}}
% single bar isomorphism
%\def\iso{\mathrel{\mathpalette\@vermin\sim}} % congruence sign
%\def\@vermin#1#2{\lower.5\p@\vbox{\baselineskip\z@skip\lineskip-3\p@
%    \ialign{$\m@th#1\hfil##\hfil$\crcr#2\crcr-\crcr}}}
\def\iso{\cong}
\def\choice#1#2{{{#1}\choose{#2}}}

\def\longdash{\hspace{1.5pt}---\hspace{1.5pt}\ignorespaces}


==> Mhdr.tex <==
% Draught style page headers: header format is:
%
% <time> <date>                <title>                <page>
% -------------------------------------------------------------
%
% where <title> is set by \title{<title>}
%
\def\ps@draught{
   \title{}
   \def\@headline{\vbox to 0pt{\vss
       \@@line{\vbox to 8.5pt{}
               \sl Draught @ \timeofday\,\tersetoday\qquad\hfil\hbox{\@title}
               \hfil\thepage}
       \vskip 4pt\hrule\vskip 4pt\vss}\hss}
   \def\@oddhead{\protect\@headline}
   \def\@evenhead{\protect\@headline}
   \def\@oddfoot{}
   \def\@evenfoot{}
   \def\sectionmark##1{}
   \def\subsectionmark##1{}}

% Paper style page headers: header format is:
%
% Even pages:
%
% <page>                                              <title> 
% -------------------------------------------------------------
%
% Odd pages:
%
% <author>                                            <page> 
% -------------------------------------------------------------
%
% where <title> is set by \title{<title>}
%
\def\ps@paper{
   \def\@oddheadline{%
       \ifnum\c@page=1 {\vbox to 0pt{}\hss}
       \else {\vbox to 0pt{\vss%
       \@@line{\vbox to 6.5pt{}\small\sl\@author\hfil\small\sl\thepage}%
       \vskip 4pt\hrule\vskip 4pt\vss}\hss}\fi}
   \def\@evenheadline{\vbox to 0pt{\vss
       \@@line{\vbox to 6.5pt{}\small\sl\thepage\hfil\hbox{\small\sl\@title}}
        \vskip 4pt\hrule\vskip 4pt\vss}\hss}
   \def\@oddhead{\protect\@oddheadline}
   \def\@evenhead{\protect\@evenheadline}
   \def\@oddfoot{}
   \def\@evenfoot{}
   \def\sectionmark##1{}
   \def\subsectionmark##1{}}

\def\ps@sicomp{
   \def\@oddheadline{%
       \ifnum\c@page=1 {\hbox to 0pt{}\hss}
       \else {\hbox to 0pt %
               {\centerline{\toupper\@author}\hss}\thepage\hss}\fi}
   \def\@evenheadline{%
       \hbox to 0pt{\centerline{\toupper\@title}\hss}%
       \hbox{}\hfill\thepage\hss}
   \def\@oddhead{\protect\@oddheadline}
   \def\@evenhead{\protect\@evenheadline}
   \def\@oddfoot{}
   \def\@evenfoot{}
   \def\sectionmark##1{}
   \def\subsectionmark##1{}
   \setlength{\textwidth}{160mm}
   \setlength{\textheight}{230mm}
   \setlength{\oddsidemargin}{6mm}
   \setlength{\evensidemargin}{-1mm}
   \setlength{\topmargin}{-10mm}
   \setlength{\headsep}{20pt}
}

\def\ps@simpap{
   \def\@oddheadline{
       \ifnum\c@page=1 \vbox to 8.5pt{} \hss
       \else 
       \@@line{\vbox to 8.5pt{}\hfil\thepage}\hss\fi}
   \def\@evenheadline{
       \@@line{\vbox to 8.5pt{}\thepage\hfil}\hss}
   \def\@oddhead{\kern-3pt\protect\@oddheadline}
   \def\@evenhead{\kern-3pt\protect\@evenheadline}
   \def\@oddfoot{}
   \def\@evenfoot{}
   \def\sectionmark##1{}
   \def\subsectionmark##1{}}

% Lecture notes style page headers: page header style is as follows:
%
% page 1 looks like:
% -------------------------------------------------------------------
%                        <course title>
% Lecturer: <lecturer>   No. <no>: <date>            Scribe:<scribe>
% -------------------------------------------------------------------
%
% all other pages look like:
%                                               No. <no>, Page <page>
%
% The various parameters are set by the following commands:
%
%   \def\coursetitle{???}   % Set this to the course number and title.
%   \def\lecturedate{???}   % Set this to the date of lecture.
%   \def\lectureno{???}     % Set this to the lecture number.
%   \def\lecturer{???}      % Set this to the name of the lecturer.
%   \def\scribe{???}        % Set this to the name of the scribe.
%

\def\ps@lecnotes{
   \def\coursetitle{$\langle\mbox{\it Course Title}\rangle$}
   \def\lecturedate{$\langle\mbox{\it Date}\rangle$}
   \def\lectureno{$\langle\mbox{\it Number}\rangle$}   
   \def\lecturer{$\langle\mbox{\it Lecturer}\rangle$}
   \def\scribe{$\langle\mbox{\it Scribe}\rangle$}
   \def\@headline{
       \ifnum\c@page=1
           \vbox to 0pt{\vss\hrule
                \vskip 4pt
                \@@line{\vrule height8.5pt depth 3.5pt width 0pt\@headertop}
                \vskip 2pt 
                \@@line{\vbox to 8.5pt{}\@headerbottom}
                \vskip 5pt\hrule\vskip 12pt\vss}
       \else 
           \vbox to 0pt{\vss\vskip 17.5pt
           \@@line{\vbox to 8.5pt{}\hfil Lecture \lectureno,\, Page \thepage}
           \vss}
       \fi\hss}
   \def\@headertop{\hfil\coursetitle\hfil}
   \def\@headerbottom{\rlap{Speaker: \lecturer}\hfil Lecture \lectureno\,:
                     \lecturedate\hfil\llap{Scribe: \scribe}}
   \def\@oddhead{\protect\@headline}
   \def\@evenhead{\protect\@headline}
   \def\@oddfoot{}
   \def\@evenfoot{}
   \def\sectionmark##1{}
   \def\subsectionmark##1{}
   \textheight 8.9in
   \textwidth 6.5in
   \marginparwidth 0pt
   \oddsidemargin 0pt
   \evensidemargin 0pt
   \topmargin -29pt
   \parindent=20pt
   \parskip=1ex plus 2pt minus 2pt
}


\if@twoside
  \def\ps@springer{
    \mark{{}{}}
    \def\@oddfoot{}
    \def\@evenfoot{}%
    \def\@evenhead{\sl\thepage\hfil\leftmark}
    \def\@oddhead{\hbox{}\sl\rightmark \hfil\thepage}
    \def\sectionmark##1{}%
    \def\subsectionmark##1{}}
\else 
  \def\ps@springer{
    \mark{{}{}}
    \def\@oddfoot{}
    \def\@evenfoot{}
    \def\@oddhead{\hbox{}\sl \rightmark \hfil \rm\thepage}
    \def\sectionmark##1{\markright{\uppercase{\ifnum \c@secnumdepth >\z@%
    \thesection\hskip 1em\relax \fi ##1}}}}
\fi

\def\today{\ifcase\month\or
 January\or February\or March\or April\or May\or June\or
 July\or August\or September\or October\or November\or December\fi
 \space\number\day, \number\year}

\ps@headings \pagenumbering{arabic} \onecolumn
\if@twoside\else\raggedbottom\fi


\newcount\mn \newcount\hr
\def\timeofday{
%  \message{time=\number\time}
  \hr=\time \divide\hr 60
  \mn=-\hr \multiply\mn 60 \advance\mn \time
  \ifnum\hr=0
     {12\,:\,\twodigits\mn\,am}
  \else{
     \ifnum\hr<13
        {\number\hr\,:\,\twodigits\mn\,am}
     \else
        {\advance\hr -12 \number\hr\,:\,\twodigits\mn\,pm}
     \fi}
  \fi}
\def\twodigits#1{\ifnum #1<10 0\fi \number#1}
\def\tersetoday{\ifcase\month\or
  Jan.\or Feb.\or Mar.\or Apr.\or May\or June\or
  July\or Aug.\or Sep.\or Oct.\or Nov.\or Dec.\fi
  \space\number\day, \number\year}

% Thesis style page headers: header format is:
%
% Even pages:
%
% <page>                                         Section  cc.ss
% -------------------------------------------------------------
%
% Odd pages:
%
% <Chapter name>                                      <page>
% -------------------------------------------------------------
%
% where <title> is set by \title{<title>}
%
\def\ps@thesis{
   \def\@oddheadline{
       \@@line{\vbox to 8.5pt{}\small\sl Section \thesection\hfil\thepage}\hss}
   \def\@evenheadline{
       \@@line{\vbox to 8.5pt{}\small\thepage\hfil\sl\@chaptername}\hss}
   \def\@oddhead{\kern-3pt\protect\@oddheadline}
   \def\@evenhead{\kern-3pt\protect\@evenheadline}
   \def\@oddfoot{}
   \def\@evenfoot{}
   \def\sectionmark##1{}
   \def\subsectionmark##1{}}


==> toc2.tex <==
\vfill
\eject
\quad
\vskip .9 in
\line{\bigbf Table of Contents\hfil}
\bigskip

{\obeylines
Introduction \dotfill 11

Chapter 1. Polynomial Decomposition \dotfill 17
\qquad A. Definition of the Problem \dotfill 17
\qquad B. Decomposition and the Subfields of $F(x)$ \dotfill 21
\qquad C. Separated Polynomials \dotfill 24
\qquad D. Multidimensional Block Decompositions \dotfill 26
\qquad E. Chebyshev Polynomials \dotfill 31
\qquad F. Complete Rational Decompositions \dotfill 34
\qquad G. The Number of Indecomposable Polynomials \dotfill 36
\qquad H. Multivariate Decomposition  \dotfill 38

Chapter 2. Decomposition Algorithms \dotfill 41
\qquad A. The Model of Computation  \dotfill 42
\qquad B. Computing Right Division  \dotfill 42
\qquad C. Univariate Decomposition Using Separated Polynomials \dotfill 44
\qquad D. Univariate Decomposition in the Tame Case \dotfill 45
\qquad E. Decomposition Using Block Decomposition \dotfill 46
\qquad F. A Lower Bound on the Degree of Splitting Fields \dotfill 48
\qquad G. Decompositions Corresponding To Ordered Factorisations \dotfill 51
\qquad H. Computing Complete Univariate Decompositions  \dotfill 53
\qquad I. Decomposition Multivariate Polynomial in the Tame Case \dotfill 53
\qquad J. Multivariate Decomposition using Separated Polynomials \dotfill 56

Chapter 3. Additive Polynomials \dotfill 59
\qquad A. Definition and Root Structure of Additive Polynomials \dotfill 59
\qquad B. Rationality and the Kernel \dotfill 63
\qquad C. Rational Decompositions of Additive Polynomials \dotfill 64
\qquad D. The Number of Bidecompositions of a Polynomial  \dotfill 65
\qquad E. Complete Decompositions of Additive Polynomials \dotfill 67
\qquad F. The Number of Complete Rational Normal Decompositions \dotfill 67

Chapter 4. The Ring of Additive Polynomials \dotfill 73
\qquad A. Basic Ring Structure  \dotfill 73
\qquad B. The Euclidean Scheme  \dotfill 75
\qquad C. The Structure of the Set of Decompositions \dotfill 80
\qquad D. Completely Reducible Additive Polynomials  \dotfill 89
\qquad E. The Uniqueness of Transmutation \dotfill 92
\qquad F. The Number of the Complete Decompositions \dotfill 95

Chapter 5. Decomposing Additive Polynomials \dotfill 96
\qquad A. The Model of Computation  \dotfill 96
\qquad B. The Cost of Basic Operations in $\ap$ \dotfill 97
\qquad C. The Minimal Additive Multiple \dotfill 98
\qquad D. Complete Rational Decomposition of Additive Polynomials \dotfill 100
\qquad E. General Rational Decomposition of Additive Polynomials \dotfill 103
\qquad F. General Decomposition of Completely 
~~~~~~~~~~Reducible Additive Polynomials \dotfill 106
\qquad G. Determining Transmutations of Additive Polynomials \dotfill 111
\qquad H. Bidecomposition of Similarity Free Additive Polynomials \dotfill 113
\qquad I. Absolute Decompositions of Additive Polynomials \dotfill 119

Chapter 6.  Rational Function Decomposition \dotfill 121
\qquad A. The Normalised Decomposition Problem \dotfill 121
\qquad B. Decomposing Normalised Rational Functions \dotfill 128

Conclusion. \dotfill 133

References.  \dotfill 135
}
\vfill
\eject


